CoFHEE: A Co-processor for Fully Homomorphic Encryption Execution (Extended Version)

The migration of computation to the cloud has raised concerns regarding the security and privacy of sensitive data, as their need to be decrypted before processing, renders them susceptible to potential breaches. Fully Homomorphic Encryption (FHE) serves as a countermeasure to this issue by enabling computation to be executed directly on encrypted data. Nevertheless, the execution of FHE is orders of magnitude slower compared to unencrypted computation, thereby impeding its practicality and adoption. Therefore, enhancing the performance of FHE is crucial for its implementation in real-world scenarios. In this study, we elaborate on our endeavors to design, implement, fabricate, and post-silicon validate CoFHEE, a co-processor for low-level polynomial operations targeting Fully Homomorphic Encryption execution. With a compact design area of $12mm^2$, CoFHEE features ASIC implementations of fundamental polynomial operations, including polynomial addition and subtraction, Hadamard product, and Number Theoretic Transform, which underlie most higher-level FHE primitives. CoFHEE is capable of natively supporting polynomial degrees of up to $n = 2^{14}$ with a coefficient size of 128 bits, and has been fabricated and silicon-verified using 55nm CMOS technology. To evaluate it, we conduct performance and power experiments on our chip, and compare it to state-of-the-art software implementations and other ASIC designs.

==> 3.1_operation.tex <==
\section{Scheduling Data \& Computation}

\cofhee{} is designed to support polynomial degrees of up to $2^{14}$ in powers of two and modulus size up to 128 bits, while it is optimized to work with a polynomial degree $n = 2^{13}$.
These values offer a trade-off between maximizing performance of FHE applications \cite{kim2015private, dowlin2016cryptonets, 10.1145/3133956.3134061, pmt, gursoy} and minimizing \cofhee{}'s area.

As \cofhee{} is a co-processor for the acceleration of polynomial multiplication, it has to support all the required high-level operations.
These operations can be divided into two types: compute operations and memory operations.
\underline{Compute operations} are NTT, inverse NTT, and a set of pointwise operations, namely: Normal and modular multiplication, modular squaring, modular multiplication by a constant, and modular addition and subtraction.
\cofhee{} provides an ISA to execute any of these operations when relevant polynomials are loaded into the memory.
Meanwhile, \underline{memory operations} copy the data from one memory to another.
Although compute operations run sequentially similar to memory operations, both types can run simultaneously.
The operations supported by \cofhee{} are listed in Table .

% \subsection{Memory vs. compute}

% \hl{The chip area available for \cofhee{}'s design is $12mm^2$, which is quite limited.
% As the FHE application performs operation on big polynomial with large coefficient size, \cofhee{} needs a large area to perform operation on big numbers and store big polynomials.
% It is not possible to completely fit all the required operands in this chip to perform any real-world application.
% Hence, \cofhee{} only stores subset of data to perform computationally intensive operations.

% We select to perform ciphertext multiplication on \cofhee{} without any interaction from an external interface, as ciphertext multiplication is the slowest FHE operation.
% Ciphertext multiplication requires four polynomials and twiddle factors as input.
% Hence, it requires five memories to store the input data.
% Ciphertext multiplication also requires two memories to store internal calculations.
% The size of each of this memory is shown in Table .
% Total memory area is the sum of dual-port memories, single-port memories for storing the data, and for loading ARM instructions.
% This totals to around $9.8 mm^2$.
% In the remaining area, we fit Processing Elements (PE), Multiplier Data Mover and Controller (MDMC), Direct Memory Access controller (DMA), General Purpose Configuration registers (GPCFG), and an ARM Cortex-M0 with its own memory.
% Table  shows a representative subset of the 35 Configuration Registers in \cofhee{}.
% Our configuration registers map to the 0x4002\_0000 -- 0x4002\_FFFF memory range.
% In our design, the memory base address follows the ARM Cortex M series memory map convention for memory and peripheral addresses.}

% For the design area available, we opted for a system architecture with 1 PE, 3 dual-port and 5 single-port SRAMs.
% This selection of units enables support of ciphertext multiplication fully on chip.
% In addition, dual-port memories enable computation with an Initiation Interval $II=1$ clock cycle.
% $II$ is defined as the number of clock cycles needed to feed new operands to the computation units.
% If the polynomial coefficients are stored in a single-port SRAM, we cannot fetch two operands and store another two operands in the same cycle.
% Hence, we choose to use dual-port SRAMs as it is possible to fetch/write two operands per memory in the same cycle at a cost in area.
% Dual-port SRAMs takes almost 2 times the area compared to single-port SRAMs.
% Therefore, we limit the number of dual-port SRAMs to three, as two are required for computation to enable loading of operands and storing of the results in the same cycle, and one serves as a buffer for loading the next polynomial to go under NTT.
% DMA is used to move the next polynomial from a single-port SRAM to the third dual-port memory while NTT is happening, adding no extra latency.}

% \subsection{Execution modes}
% \hl{There are three ways to execute the basic operations supported by \cofhee{} (Table ):
% 1) The simplest option is for the external host to directly trigger the MDMC to perform the commands through a configuration register write.
% This mode is slow as there are delays imposed by the communication interface when writing to the configuration register.
% 2) Another possibility is to use the command FIFO, where the external host preloads the sequence of commands to be executed and waits for an interrupt issued by \cofhee{} signaling that the queue is empty.
% As soon as the first command is written to the queue, the command FIFO sends it to the MDMC.
% The MDMC starts the operation and once it completes, it sends a signal to the command FIFO.
% The process repeats until all commands have been executed.
% The command FIFO guarantees the execution of a single command at a time in a predefined order.
% Thus, it requires less control logic and avoids complicated  out-of-order executions.
% In addition, the command FIFO gives the flexibility to execute different complex operations as combinations of basic instructions. 
% %As an example, one can load a sequence of commands to perform a ciphertext multiplication.
% We defined the length of the queue to be 32 commands, as it is more than sufficient for our target applications. 
% %Whenever the command FIFO becomes empty, the external host has to load another set of commands.
% %This can be time consuming depending on the external host interface speed.
% The host can continuously load more commands while the queue is not full. 
% 3) For a faster and flexible sequencing and execution of commands, we introduce a third mode, which utilizes a 32-bit ARM Cortex M0 (CM0) along with a dedicated instruction memory.
% In this mode, the processor is used instead of the command FIFO.
% One can write complex subroutines and sequence of operations in embedded C, then compile and preload it in CM0's instruction memory for later execution.}

==> 3_method_old.tex <==
% The architecture consists of .... . A detailed description of each main component is provided in the following sections. 

\section{\cofhee{} Design Flow Overview}
\label{sec:method}
% \newpage

\subsection{Ciphertext Multiplication}
\label{sss:ctmul}


The most computationally intense low-level FHE operation is the ciphertext multiplication. Consequently, the main objective of the \cofhee{} co-processor is native support for modular operations, which is essential for accelerating FHE cryptosystems. \cofhee{} is designed to support polynomial degrees of up to $2^{14}$ in powers of two and modulus size up to 128 bits, while it is optimized to work with a polynomial degree $n = 2^{13}$.
These values offer a trade-off between maximizing performance of FHE applications \cite{kim2015private, pmt, gursoy} and minimizing \cofhee{}'s area.


\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs/toparch.png}
    \includegraphics[width=\linewidth]{figs/toparch_DATE.png}
    \caption{\cofhee{}~Top Level Architecture} 
    % Remake Diagram
    \label{fig:TopArch}
    % \vspace{-1cm}
\end{figure}



\cofhee{}'s design is constrained by a limited chip area of $12mm^2$ and the use of $55nm$ CMOS technology from GlobalFoundries. Given the aforementioned limitations and the common encryption parameters used in FHE applications (Section \ref{sss:ctmul}), we have determined that the maximum polynomial degree that can be supported on the chip is $n=2^{13}$, with coefficient sizes of 128 bits. This is the largest coefficient size that can be accommodated within the design area constraints. In the case of $n=2^{14}$, extra communication is required. To achieve this goal, we have developed a system architecture that includes 1 Processing Element (PE), 3 dual-port and 5 single-port SRAMs. This configuration of units allows for full on-chip ciphertext multiplication with an Initiation Interval ($II$) of 1, as the dual-port SRAMs enable the simultaneous fetching and storing of 2 different operands in the same cycle. \hl{We utilized dual-port memory as opposed to using two separate single-port memories. This decision not only minimized the overall area (given that a single dual-port memory occupies less space than two equivalent single-port memories), but also streamlined the design of the controller.} The majority of the available chip area is occupied by the SRAMs, with the remaining space allocated for the PEs, Multiplier Data Mover and Controller (MDMC), Direct Memory Access controller (DMA), General Purpose Configuration registers (GPCFG), and an ARM Cortex-M0 processor with its own memory. Additionally, the chip operates at a target frequency of $250$ MHz, which is limited by the memory latency, and has two voltage supplies, $3.3$ V for the IO pads and $1.2$ V for the logic core. Table \ref{tab:gpcfg} shows a representative subset of the 35 Configuration Registers in \cofhee{}. The configuration registers in CoFHEE are mapped to the memory range of 0x4002 0000 – 0x4002 FFFF, and the chip's memory base address follows the ARM Cortex M series memory map convention for memory and peripheral addresses. \hl{By assigning unique base addresses to each port of the dual-port memories, we treat them as separate address spaces at the bus level. This approach circumvents complications in the MDMC, which would otherwise have to identify the type of memory being accessed.}

% The chip area available for \cofhee{}'s design is $12mm^2$ and the available technology node is GF $55nm$. Considering this limitation in area, and common encryption parameters used in FHE applications (Section \ref{sss:ctmul}), we can achieve our goal of performing ciphertext multiplication on chip for a maximum polynomial degree $n=2^{13}$ with 128-bit coefficient sizes (in case of $n=2^{14}$, extra communication is needed).
% A 128-bit coefficient size is the largest coefficient we can fit in \cofhee{} given design area limitations. The aforementioned restrictions allowed us to develop a system architecture with 1 Processing Element (PE), 3 dual-port and 5 single-port SRAMs. 
% This selection of units enables support of ciphertext multiplication fully on chip, with an $II$ (Initiation Interval) $=1$, as the dual-port SRAMs provide the ability to fetch and store 2 different operands in the same cycle. 
% The biggest portion of the provided area is occupied by the dual and single-port SRAMs. In the remaining space, we fit the Processing Elements (PE), Multiplier Data Mover and Controller (MDMC), Direct Memory Access controller (DMA), General Purpose Configuration registers (GPCFG), and an ARM Cortex-M0 with its own memory. Table \ref{tab:gpcfg} shows a representative subset of the 35 Configuration Registers in \cofhee{}.
% Our configuration registers map to the 0x4002\_0000 -- 0x4002\_FFFF memory range.
% In our design, the memory base address follows the ARM Cortex M series memory map convention for memory and peripheral addresses. Lastly, the chip operates at a target frequency of $250$ MHz (bounded by the memory latency), and has two voltage supplies, namely $3.3$ V (IO pads) and $1.2$ V (logic core).

% \begin{figure}[ht!]
%     % \hspace{0.2cm}
%     \begin{minipage}[t][][t]{0.32\textwidth}
%         \centering
%         \input{tables/gpcfg}
%     \end{minipage}
% \end{figure}
% % Ciphertext multiplication requires four polynomials and twiddle factors as input.
% % Hence, it requires five memories to store the input data.
% It is important to note that dual-port memories play a crucial role in our design. Dual-port memories enable computation with an Initiation Interval $II=1$ clock cycle.
% $II$ is defined as the number of clock cycles needed to feed new operands to the computation units.


% If the polynomial coefficients are stored in a single-port SRAM, we cannot fetch two operands and store another two operands in the same cycle.
% Hence, we choose to use dual-port SRAMs as it is possible to fetch/write two operands per memory in the same cycle at a cost in area.
% Dual-port SRAMs takes almost 2 times the area compared to single-port SRAMs.
% Therefore, we limit the number of dual-port SRAMs to three, as two are required for computation to enable loading of operands and storing of the results in the same cycle, and one serves as a buffer for loading the next polynomial to go under NTT.
% DMA is used to move the next polynomial from a single-port SRAM to the third dual-port memory while NTT is happening, adding no extra latency.


% The chip area available for \cofhee{}'s design is $12mm^2$, which is quite limited.
% As the FHE application performs operation on big polynomial with large coefficient size, \cofhee{} needs a large area to perform operation on big numbers and store big polynomials.
% It is not possible to completely fit all the required operands in this chip to perform any real-world application.
% Hence, \cofhee{} only stores subset of data to perform computationally intensive operations.

% We select to perform ciphertext multiplication on \cofhee{} without any interaction from an external interface, as ciphertext multiplication is the slowest FHE operation.
% Ciphertext multiplication requires four polynomials and twiddle factors as input.
% Hence, it requires five memories to store the input data.
% Ciphertext multiplication also requires two memories to store internal calculations.
% The size of each of this memory is shown in Table .
% Total memory area is the sum of dual-port memories, single-port memories for storing the data, and for loading ARM instructions.
% This totals to around $9.8 mm^2$.
% In the remaining area, we fit Processing Elements (PE), Multiplier Data Mover and Controller (MDMC), Direct Memory Access controller (DMA), General Purpose Configuration registers (GPCFG), and an ARM Cortex-M0 with its own memory.
% Table  shows a representative subset of the 35 Configuration Registers in \cofhee{}.
% Our configuration registers map to the 0x4002\_0000 -- 0x4002\_FFFF memory range.
% In our design, the memory base address follows the ARM Cortex M series memory map convention for memory and peripheral addresses.}


% \hl{Fig. \ref{fig:TopArch} shows \cofhee{}'s top architecture.}
% \hl{The PE is connected to the MDMC, which in turn has a direct connection to the command FIFO and communicates with the memories using the AHB lite interconnect.
% The AHB lite interconnect connects all IPs and ensures reliable data movement with variable data sizes.
% The MDMC performs memory reads and writes for computation; DMA transfer data from one memory to another; and the external interfaces communicate with the host.}

% \subsection{Clock frequency}

% \cofhee{}'s frequency is defined by the critical path of the design as well as the technology node targeted.
% The critical path can be either in the computation unit due to a complex data path or it can be in the memory as a consequence of memory read latency.
% While the former can be reduced with pipelining, memory read latency is fixed for the technology node and memory size used.
% As expected, \cofhee{}'s critical path is in the memory read for loading data from the memory to the computation unit.
% For the technology node targeted, i.e., Globalfoundries (GF) 55nm low power enhanced (LPE) process, the memory read path is around $4ns$, which translates to a clock frequency of 250 Mhz.
% %A 22nm TSMC memory compiler \cite{noauthor_synopsys_memcomp} reports the memory read latency to be around 1.4 ns, meaning that \cofhee{} can easily reach 600-700 Mhz or higher frequencies if implemented in this technology node.

\subsection{Execution \& Operations}
\setcounter{page}{3}
\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs/toparch.png}
    \includegraphics[width=\linewidth]{figs/steps.png}
    \caption{Execution flow of operations} 
    % Remake Diagram
    \label{fig:ExecFlow}
    % \vspace{-1cm}
\end{figure}

% \input{tables/operations}

% \cofhee{} is designed to support polynomial degrees of up to $2^{14}$ in powers of two and modulus size up to 128 bits, while it is optimized to work with a polynomial degree $n = 2^{13}$.
% These values offer a trade-off between maximizing performance of FHE applications \cite{kim2015private, pmt, gursoy} and minimizing \cofhee{}'s area.

%  dowlin2016cryptonets, 10.1145/3133956.3134061

%As  is a co-processor for the acceleration of polynomial multiplication, it has to support all the fundamental operations.
% \cofhee{} supported operations can be divided into two types: Compute and memory operations.
% Compute operations consist of NTT, inverse NTT, and a set of pointwise operations, namely normal and modular multiplication, modular squaring, modular multiplication by a constant, and modular addition and subtraction.
% \cofhee{} provides an ISA to execute any of these operations when relevant polynomials are loaded into the memory.
% Meanwhile, memory operations replicate or transfer data from one memory to another.
% Although compute operations run sequentially similar to memory operations, both types can run simultaneously.
\cofhee{} supports a range of operations that can be broadly classified into two categories: compute and memory operations. Compute operations include the Number Theoretic Transform (NTT), Inverse Number Theoretic Transform (INTT), and a set of pointwise operations such as normal and modular multiplication, modular squaring, modular multiplication by a constant, and modular addition and subtraction. \cofhee{} provides an Instruction Set Architecture (ISA) to execute any of these operations when the relevant polynomials are loaded into the memory. On the other hand, memory operations include the replication or transfer of data from one memory to another. While compute operations run in a sequential manner, memory operations can be run simultaneously, which allows for concurrent execution of both types of operations.
The operations supported by \cofhee{} are summarized in Table \ref{tab:basic_ops}.

\input{tables/gpcfg}


% \subsubsection{Modular Multiplication}
% Modular multiplication involves normal multiplication followed by a modular reduction of the product. There are few prominent types of modular multiplication; interleaved, Barrett, and Montgomery \cite{cryptohandbook}. 
% Barrett is selected for our implementation as there is no need to transform the arguments, as required for Montgomery \cite{modmulalgocomp}. It has an $II = 1$ and
% the target frequency can be achieved by pipelining a single Barrett design whereas for the interleaved multiplier, to achieve $II$ of $1$, one needs to increase the number of said multipliers linearly, thus increasing the design area as well as the number of nets in the design.

% \input{tables/operations}


% \subsubsection{Algorithms}
\textit{Algorithms}:
% There are few prominent types of modular multiplication; interleaved, Barrett, and Montgomery \cite{cryptohandbook}. 
% Barrett is selected for our implementation as there is no need to transform the arguments, as required for Montgomery \cite{modmulalgocomp}. 
Regarding polynomial multiplication, \cofhee{} implements and operates using the Cooley-Tukey NTT algorithm \cite{cooley-tukey}.
\cofhee{} also handles a ciphertext multiplication algorithm. 
% Algorithm \ref{alg:ctmul} describes the ciphertext multiplication operation as handled by \cofhee{}.
Two ciphertexts (polynomial pairs) are passed as input.
The ciphertext polynomials are multiplied following Eq. \ref{eq:ctmul}. 
Each polynomial is used twice in polynomial multiplications.
Nevertheless, we only need one NTT operation per polynomial as they can stay in the NTT domain during the polynomial multiplication and addition.
At the end, we can convert back from the NTT domain using the iNTT operation.
The entire ciphertext multiplication in \cofhee{} utilizes 4 NTTs, 4 Hadamard products, 1 pointwise addition, and 3 iNTTs.

\hl{Regarding execution, when executing a command such as NTT, an internal state machine within the MDMC is activated. This state machine is responsible for managing data transfers: specifically, it relocates data from the memory to the processing element (PE) and subsequently transfers the PE's computation results back to the memory.

The state machine also handles the incrementation of addresses for both operands and twiddle factors, although the twiddle factors themselves don't undergo an address increment. The decision regarding how the address is incremented is contingent upon the current stage of the NTT operation. Once a stage is finalized, the MDMC processes the output, subsequently initiating the subsequent stage.
Once the computational operation reaches completion, an interrupt is generated, prompting the command first-in-first-out (FIFO) buffer to issue the succeeding instruction. }Figure \ref{fig:ExecFlow} provides an illustration of the execution flow of the proposed method.

% \input{algo/ctmul}
% \begin{figure}[ht!]
%     % \begin{minipage}[t][][t]{0.46\textwidth}
%     %     \centering
%     %     \input{algo/ntt}
%     %     \vspace{-0.5cm}
%     %     \input{algo/polymul}
%     % \end{minipage}
%     % \hspace{0.2cm}
%     \begin{minipage}[t][][t]{0.46\textwidth}
%         \centering
%         \input{algo/ctmul}
%     \end{minipage}
% \end{figure}

\subsection{\cofhee{} API}

\cofhee{} exposes assembly-like instructions for the operations listed in Table \ref{tab:basic_ops}.
Composed operations such as polynomial multiplication or ciphertext multiplication build on top of the atomic ones. 
\cofhee{}'s design is optimized for $n=2^{13}$.
Nevertheless, it supports any $n \leq 2^{14}$, assuming that $n$ is a power of two.
It can perform NTT, polynomial multiplications, and ciphertext multiplications on chip with $II=1$, without requiring back-and-forth communication to the host during the computation for any $n \leq 2^{13}$.
In the case of $n=2^{14}$, \cofhee{} can perform NTT on chip with $II=2$, as single-port memories need to be used for computation. \hl{However, while polynomial multiplications and ciphertext multiplications are also possible, they require back-and-forth data movement with the host, as it is not possible to fit all data at once on chip. Larger polynomials ($n > 2^{14}$) on the other hand are too large even for the NTT operation and, therefore, \cofhee{} does support them.
Nevertheless, such larger polynomials are not commonly used in FHE application due to their higher overheads.}
%, while polynomial and ciphertext multiplications require back-and-forth communication.

The maximum coefficient size supported by \cofhee{} is 128 bits.
Additions and subtractions take 1 cycle and multiplication takes 4 cycles, independently of the coefficient size.
Coefficients larger than 128 bits must be broken using RNS, similarly to how it is done in software, to fit in \cofhee{}. \hl{The reason we selected an 128-bit coefficient size is related to the complexity of the key-switching operation. While RNS enables the split of a large modulus polynomial into several smaller modulus towers or limbs, increasing the number of RNS towers also elevates the complexity during key switching. Therefore, accommodating a larger modulus size allows for fewer RNS towers, resulting in a simpler key switching process.}

\input{tables/operations}

\subsection{Clock frequency}

\cofhee{}'s frequency is defined by the critical path of the design as well as the technology node targeted.
The critical path can be either in the computation unit due to a complex data path or it can be in the memory as a consequence of memory read latency.
While the former can be reduced with pipelining, memory read latency is fixed for the technology node and memory size used.
As expected, \cofhee{}'s critical path is in the memory read for loading data from the memory to the computation unit.
For the technology node targeted, i.e., Globalfoundries (GF) 55nm low power enhanced (LPE) process, the memory read path is around $4ns$, which translates to a clock frequency of 250MHz.
%A 22nm TSMC memory compiler \cite{noauthor_synopsys_memcomp} reports the memory read latency to be around 1.4 ns, meaning that \cofhee{} can easily reach 600-700 Mhz or higher frequencies if implemented in this technology node.


% \vspace{-0.1cm}
\subsection{Processing Element}
% \subsubsection{Processing Elements (PEs)}
% A processing element is a basic processing unit.
\hl{\cofhee{} comprises a singular modular multiplier, along with modular adder and subtractor units. Furthermore, the processing element encompasses a series of multiplexers (MUXs) designed to direct operands and intermediate data, depending on whether the operation involves multiplication, addition, or subtraction within the utilized butterfly structure. This enables the processing element to function as a versatile unit for NTT and iNTT operations, as well as element-wise additions, subtractions, and multiplications.

Surrounding the processing element, we have implemented a wrapping logic that orchestrates the movement of data from memory to the processing element, tailored to the specific operation at hand, whether it's NTT, iNTT, or element-wise operations. In the context of NTT and iNTT, the processing element essentially serves as a singular radix-2 butterfly NTT unit.
}

% \hl{\cofhee{} is composed of a single modular multiplier, one modular adder, and one modular subtractor units. In addition, the processing element contains a number of MUXs to route the opernds and intermediate data based on whether the operation is multiplication, addition, subtraction of the utilized butterfly structure. This allows for the processing element to be used as unit for the NTT and iNTT operations as well as element-wise additions subtractions and multiplications. We have implemented a wrapper logic around the processing element that moves the data from memory to the processing element according to the operation that needs to be performed (between NTT, iNTT, and element-wise operations). Regarding NTT and iNTT, essentially, the processing element acts as a single radix-2 butterfly NTT unit. }
\cofhee{}'s PE supports modular multiplication, modular addition, and modular subtraction.
Each operation has an $II=1$.
Modular addition and subtraction have a latency of one clock cycle, while modular multiplication completes in five clock cycles.
In contrast to the state-of-the-art that uses Montgomery multipliers, \cofhee{} employs a Barrett multiplier to implement multiplication and modular reduction due to its pipelining capabilities \cite{modmulalgocomp}. \hl{We chose to use Barrett reduction instead of Montgomery reduction based on our design space exploration on these two multipliers. Barrett reduction offers a better tradeoff between power, performance, and area (PPA), and it is also easier to pipeline for achieving higher frequencies.} The pipeline depth is chosen such that the critical path matches the memory read latency. 
%In addition, a Barrett multiplier enables normal multiplication as it is possible to bypass the modular reduction at the end.
Our PE operates in four distinct modes defined by the mode selection input.
The operations modes are: (1) Modular Multiplication, (2) Modular Addition, (3) Modular Subtraction, and (4) Butterfly operation.
The butterfly operation is an atomic computational unit of NTT.
It is executed by performing modular multiplication followed by modular addition and modular subtraction.
We implement the butterfly operation using radix 2, and acquire a PE that occupies $6\%$ of the design area.
% Using the four modes, \cofhee{}'s PE executes all compute operations mentioned in Table \ref{tab:basic_ops} while occupying 6\% of the design area.
% Normal and modular multiplication, as well as modular squaring work on mode (1).
% Different bits in the operation command set flags to, for example, bypass the modular reduction, enabling a variety of similar operations to use the same hardware.
% \vspace{-0.4cm}
\subsection{NTT considerations}
For a $2\times$ performance improvement of NTT, the input and output polynomials are stored in dual-port memories.
In addition, there is a third dual-port memory to store the next polynomial to go under NTT.
If the next polynomial is in a single-port memory, DMA is used to transfer polynomial coefficients to the available dual-port memory while NTT operates on the current polynomial.
This is possible since the bus architecture allows the MDMC, DMA, and ARM CM0 to access memories in parallel.
Once NTT completes, the dual-port memories switch tasks; the one containing the next polynomial participates in the following NTT, while the memory containing the output uses DMA to offload the result to a single-port memory and load the next polynomial for NTT.
This process happens transparently in the background without performance degradation due to data movement.

% \vspace{-0.4cm}
\subsection{Internal Data Flow}
\subsubsection{Interconnect}
We implement a parameterized Advanced High-Performance Bus (AHB) lite interconnect \cite{noauthor_amba_2001} as it supports the required bus transfer operations and has low area utilization. \hl{We chose a lightweight AHB-Lite bus for our interconnect, in contrast to most other studies that utilize AXI. The use of AXI often results in a higher signal count, which can contribute to increased routing congestion during the backend process.} \cofhee{} requires single memory transfers as well as burst memory operations, with the data sizes ranging from 32 to 128 bits. 
% \hlorange{Table}  shows a representative subset of the 35 Configuration Registers in \cofhee{}.
Our configuration registers map to the 0x4002\_0000 -- 0x4002\_FFFF memory range.
In our design, the memory base address follows the ARM Cortex M series memory map convention for memory and peripheral addresses.
% The interconnect should provide this flexibility. 
% \hl{+++}
% Explain that this creates no significant bottlenecks 

\subsubsection{Multiplier Data Mover and Controller (MDMC)}

The sequence of commands to be executed is stored in the command FIFO, which decodes the command and triggers the MDMC for the requested operation. The FIFO also provides the memory base addresses of input operands and output result.
When running computation-based operations, the MDMC fetches data from memory and forwards to the PE on every clock cycle until the operation is completed.
Once the data is processed, the MDMC stores the data back to the output memory.
% \hl{For NTT and iNTT, the MDMC needs to forward three input data and store two output data per cycle.}
In order to achieve an $II=1$ for each butterfly operation, we store the input and output polynomials in dual-port memories.
Thus, we can fetch two polynomial coefficients from one memory (dual-port) and a twiddle factor from another (single-port) in a single clock cycle.
After computing the butterfly operation, the MDMC stores the two outputs in the output memory (dual-port).
Once an NTT stage completes, the output memory acts as input memory and vice-versa, until the NTT/iNTT is finalized.
%Due to the complexity of the operations ran by the MDMC, we employ a finite state machine (FSM) which maintains internal information regarding ongoing operations.

% The MDMC performs complex operations which run for thousands of clock cycles.
% For that reason, it employs a finite state machine (FSM) to maintain internal information about the ongoing operation.
% \vspace{-0.2cm}
\subsection{External Interfaces}
% \subsubsection{IO}
\cofhee{} provides SPI and UART interfaces for external host communication.
These interfaces are used for loading polynomials, triggering the required operation and reading back the result.
SPI and UART are chosen mainly for their simplicity in implementation as well as the ability to communicate from an external PC.
One can always replace these interfaces with faster ones such as PCI-express or HSIC (High-Speed Inter-Chip).
Other IOs in \cofhee{} are clock, reset, voltage supplies, bias voltages, bias currents, PLL controls, and debugging IOs.



% \input{algo/ctmul}

% \subsection{Design Blocks}


%\subsection{Pre-silicon verification}

%We verified the functionality of our RTL design using both simulation and FPGA-based validation.
%The simulation was performed using Synopsys VCS at the top-level.
%A Python script is used to calculate the modulus following the equation $q = 2 k \cdot n + 1$, where $k \ge 1$ is an arbitrary constant.
%In addition, the script finds twiddle factors, generate random input polynomial coefficients, and calculate the expected results.
%We use random coefficient values modulo $q$ for our test polynomials since the 128-bit operand range cannot be exhaustively tested.
%These values are then ported to the Verilog testbench, where they are loaded and the result from the design is compared against the expected result.
% Once the polynomial degree $n$ is fixed, the python script finds different prime numbers in the form of $q = k*n+1$, where k is some constant, to be used as modulus. Then corresponding twiddle factors are calculated. 
% Moreover, for our FPGA design, we implemented a scaled-down version of \cofhee{}, as $n=2^{13}$ is incompatible with the available resources of our FPGAs.
% Specifically, the maximum polynomial degree that could be supported on a Digilent Nexys 4 is $n=2^{12}$ running at 10 MHz.



\subsection{Execution modes}
There are three ways to execute the basic operations supported by \cofhee{} (Table \ref{tab:basic_ops}). The simplest option is for the external host to directly trigger the MDMC to perform the commands through a configuration register write.
This mode is slow as there are delays imposed by the communication interface when writing to the configuration register.
A second possibility is to use the command FIFO, where the external host preloads the sequence of commands to be executed and waits for an interrupt issued by \cofhee{} signaling that the queue is empty.
As soon as the first command is written to the queue, the command FIFO sends it to the MDMC.
The MDMC starts the operation and once it completes, it sends a signal to the command FIFO.
The process repeats until all commands have been executed.
The command FIFO guarantees the execution of a single command at a time in a predefined order.
Thus, it requires less control logic and avoids complicated  out-of-order executions.
In addition, the command FIFO gives the flexibility to execute different complex operations as combinations of basic instructions. 
%As an example, one can load a sequence of commands to perform a ciphertext multiplication.
We define the length of the queue to be 32 commands, as it is more than sufficient for our target applications. 
%Whenever the command FIFO becomes empty, the external host has to load another set of commands.
%This can be time consuming depending on the external host interface speed.
The host can continuously load more commands while the queue is not full. Lastly, for a faster and flexible sequencing and execution of commands, we introduce a third mode, which utilizes a 32-bit ARM Cortex M0 (CM0) along with a dedicated instruction memory.
In this mode, the processor is used instead of the command FIFO.
One can write complex subroutines and sequence of operations in embedded C, then compile and preload it in CM0's instruction memory for later execution.


\subsection{Pre-silicon verification}

We verified the functionality of our RTL design using both simulation and FPGA-based validation.
The simulation was performed using Synopsys VCS at the top-level.
A python script is used to calculate the modulus following the equation $q = 2 k \cdot n + 1$, where $k \ge 1$ is an arbitrary constant.
In addition, the script finds twiddle factors, generate random input polynomial coefficients, and calculate expected results.
We use random coefficient values modulo $q$ for our test polynomials since the 128-bit operand range cannot be exhaustively tested.
These values are then ported to the verilog testbench, where they are loaded and the result from the design is compared against the expected result.
% Once the polynomial degree $n$ is fixed, the python script finds different prime numbers in the form of $q = k*n+1$, where k is some constant, to be used as modulus. Then corresponding twiddle factors are calculated. 
Moreover, for our FPGA design, we implemented a scaled-down version of \cofhee{}, as $n=2^{13}$ is incompatible with the available resources of our FPGAs.
Specifically, the maximum polynomial degree that could be supported on a Digilent Nexys 4 is $n=2^{12}$ running at 10 MHz.

\subsection{Synthesis}

% \input{tables/synthesis} % merged with table tables/area.tex

\cofhee{}'s RTL code is synthesized using a $55nm$ standard cell library from GlobalFoundries and a clock constraint of 250MHz.
SPI IO timing is constrained to meet 50MHz of interface speed.
There is no specific IO timing constraint set for UART as it is an asynchronous interface.
Following standard practices, the standard cell library used for synthesis was the one characterized for the worst voltage (1.08V), temperature (125C), resistance, and capacitance.
Synthesizing with such a library ensures that we can achieve the target frequency in various operating conditions.
For synthesis, we use the Synopsys Design Compiler (DC).
In Table \ref{tab:area}, we present the post synthesis area and timing of the major \cofhee{} blocks.
Other than memory, the largest design is the PE, followed by the AHB and configuration registers.
Post-synthesis, we observe many blocks with critical timing path much higher than the target clock period of $4ns$. This is because synthesis setup uses restricted standard cell library with no access to faster library cells such as the ones with lower threshold voltage $V_t$.
As these paths are long combinational paths, they easily meet timing in the backend, where all the standard cell libraries are used.
In this condition, paths starting from memory become the critical path due to memory read latency (around $3.1ns$). 
We verified the functionality of our RTL design using both simulation and FPGA-based validation.

% \begin{figure}[t]
%     \hspace{0.2cm}
%     % \begin{minipage}[t][][t]{0.20\textwidth}
%     %     \input{tables/io_ports}
%     % \end{minipage}
%     \begin{minipage}[t][][t]{0.50\textwidth}
%         \input{tables/area}
%     \end{minipage}
% \end{figure}

% \cofhee{} includes an additional UART interface that sends the start address of the result polynomial to the external host once the triggered operation is done.
% In addition, \cofhee{} provides an interrupt to the external host as a way of signaling the completion of the triggered operation.
% Other IOs in \cofhee{} are clock, reset, voltage supplies, bias voltages, bias currents, PLL controls, and debugging IOs.
% The clock input provides reference clock for the PLL, reset is active low asynchronous, voltage supplies for digital are 3.3V for the IO pads and 1.2V for the core standard cells and memories.

==> f1_heax_comp.tex <==
\begin{table*}[t]
    \centering
    \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{||c|c|c|c|c|c|c|c|c|c||}
        \hline
         \multirow{2}*{\bf Design} & {\bf Technology} & {\bf n} & {\bf log q*} & {\bf Area} & {\bf Power } &   {\bf Freq.} & {\bf Clock } & {\bf Efficiency} & {\bf Silicon} \\
                                {}  &       &         &    ($bits$) &   ($mm^2$ | LUT/FF/BRAM/DSP) & {\bf ($W$)}       &    ($Mhz$) &   {\bf Cycles} &   {\bf (Performance per $mm^2$)}       &   {\bf Proven}  \\ \hline \hline
           \cofhee{}                &         ASIC - GF 55$nm$ &$2^{14}$ &         128 &         12 & $2.3 \cdot 10^{-2}$                 &        250 &   24576       &    $2.60$ $\cdot$ $10^{-4}$           & \ding{108}   \\ \hline
           F1 \cite{feldmann2021f1} &      ASIC - GF 14/12$nm$ &  $2^{14}$ &         32  &      151.4 & $1.8 \cdot 10^2$               &        1000 & 16       &       $1.73$ $\cdot$ $10^{-4}$         & \ding{109}   \\ \hline
           HEAX \cite{riazi_heax}   &       FPGA - Intel Arria10 GX 1150  & $2^{14}$ &         27  &         $582148$ / $1554005$ / $3986$ / $2018$ &   -                  &       300 &  1536       &     $\dagger$           & N/A   \\ \hline
           Roy \cite{roy2019fpga}   &        Xilinx Zynq UltraScale+ ZCU102  &  $2^{12}$ &         30  &          $63522$ / $25622$ / $400$ / $200$ &   -                  &       200 & 16425       &      $\dagger$         & N/A    \\ \hline
        %   Liu \cite{liu2019optimized}   &        20  & $2^{13}$ &         27  &          - &    -                  &      333 &  33966       &      -        & -    & \ding{109}    \\ \hline
    \end{tabular}
    }
    % \vspace{1em}
    \caption{Comparative table and performance of the NTT operation against related work}
    % \caption{Performance comparison of the NTT operation against related work}
    \footnotesize{$\dagger$ No information is available to accurately map FPGA resources to silicon area }\\
    %\vspace{-0.4cm}
    \label{tab:F1_HEAX_comp}
    % \vspace{-0.4cm}
\end{table*}


% $^1$ Efficiency is measured in NTT operations per $ns$ per $mm^2$ $\cdot$ $10^{-4}$,

==> tables/clock_tree_synthesis.tex <==
\begin{table}[t]
    \centering
    \caption{Post-CTS statistics.}\label{tab:clockstat}
    \begin{tabular}{||l|r||}
         \hline
         \multirow{2}{*}{\parbox{2.0cm}{{\bf Parameter}}}                      &
         \multirow{2}{*}{\parbox{1.5cm}{\centering {\bf Value}}}                        \\
         {} & {}  \\
        %\bf{Parameter} & \bf{Value}  \\
        \hline \hline
        clock name & HCLK \\
        \hline
        CTS synthesis corner & slow \\
        \hline
        Number of levels & 26 \\
        \hline
        Number of Sinks & 18413 \\
        \hline
        Number of clock tree buffers & 464 \\
        \hline 
        Global Skew & 240 ps \\
        \hline
        Longest Insertion delay & 2.079 ns \\
        \hline
        Shortest Insertion delay & 1.838 ns \\
        \hline 
        
    \end{tabular}
\end{table}

==> tables/f1_heax_comp_old.tex <==
\begin{table*}[t]
    \centering
    \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{||c|c|c|c|c|c|c|c|c|c||}
        \hline
         \multirow{2}*{\bf Design} & {\bf Technology} & {\bf n} & {\bf log q*} & {\bf Area} & {\bf Power } &   {\bf Freq.} & {\bf Clock } & {\bf Efficiency} & {\bf Silicon} \\
                                {}  &       &         &    ($bits$) &   ($mm^2$ | LUT/FF/BRAM/DSP) & {\bf ($W$)}       &    ($Mhz$) &   {\bf Cycles} &   {\bf (Performance per $mm^2$)}       &   {\bf Proven}  \\ \hline \hline
           \cofhee{}                &         ASIC - GF 55$nm$ &$2^{14}$ &         128 &         12 & $2.3 \cdot 10^{-2}$                 &        250 &   114688       &    $2.60$ $\cdot$ $10^{-4}$           & \ding{108}   \\ \hline
           F1 \cite{feldmann2021f1} &      ASIC - GF 14/12$nm$ &  $2^{14}$ &         32  &      151.4 & $1.8 \cdot 10^2$               &        1000 & 26       &       $1.73$ $\cdot$ $10^{-4}$         & \ding{109}   \\ \hline
           CraterLake \cite{samardzic2022craterlake} &      ASIC - 14/12$nm$ &   &         28  &      472.3 & $3.2 \cdot 10^2$               &        1000 &        &                & \ding{109}   \\ \hline
           BTS \cite{kim2022bts} &      ASIC - 7$nm$ &   &         64  &      373.6 & $1.6 \cdot 10^2$               &        1200 &        &               & \ding{109}   \\ \hline
           ARK \cite{kim2022ark} &      ASIC - 7$nm$ &   &         64  &      418.3 & $2.8 \cdot 10^2$               &        1000 &        &                & \ding{109}   \\ \hline
           HEAX \cite{riazi_heax}   &       FPGA - Intel Arria10 GX 1150  & $2^{14}$ &         27  &         $582148$ / $1554005$ / $3986$ / $2018$ &   -                  &       300 &  1536       &     $\dagger$           & N/A   \\ \hline
           Roy \cite{roy2019fpga}   &        Xilinx Zynq UltraScale+ ZCU102  &  $2^{12}$ &         30  &          $63522$ / $25622$ / $400$ / $200$ &   -                  &       200 & 16425       &      $\dagger$         & N/A    \\ \hline
        %   Liu \cite{liu2019optimized}   &        20  & $2^{13}$ &         27  &          - &    -                  &      333 &  33966       &      -        & -    & \ding{109}    \\ \hline
    \end{tabular}
    }
    % \vspace{1em}
    \caption{Comparative table and performance of the NTT operation against related work}
    % \caption{Performance comparison of the NTT operation against related work}
    \footnotesize{$\dagger$ No information is available to accurately map FPGA resources to silicon area }\\
    %\vspace{-0.4cm}
    \label{tab:F1_HEAX_comp}
    % \vspace{-0.4cm}
\end{table*}


% $^1$ Efficiency is measured in NTT operations per $ns$ per $mm^2$ $\cdot$ $10^{-4}$,




% \begin{table*}[t]
%     \centering
%     \resizebox{2\columnwidth}{!}{%
%     \begin{tabular}{||c|c|c|c|c|c|c|c|c|c||}
%         \hline
%          \multirow{2}*{\bf Design} & {\bf Technology} & {\bf n} & {\bf log q*} & {\bf Area} & {\bf Power } &   {\bf Freq.} & {\bf Clock } & {\bf Efficiency} & {\bf Silicon} \\
%                                 {}  &       &         &    ($bits$) &   ($mm^2$ | LUT/FF/BRAM/DSP) & {\bf ($W$)}       &    ($Mhz$) &   {\bf Cycles} &   {\bf (Performance per $mm^2$)}       &   {\bf Proven}  \\ \hline \hline
%            \cofhee{}                &         ASIC - GF 55$nm$ &$2^{14}$ &         128 &         12 & $2.3 \cdot 10^{-2}$                 &        250 &   24576       &    $2.60$ $\cdot$ $10^{-4}$           & \ding{108}   \\ \hline
%            F1 \cite{feldmann2021f1} &      ASIC - GF 14/12$nm$ &  $2^{14}$ &         32  &      151.4 & $1.8 \cdot 10^2$               &        1000 & 16       &       $1.73$ $\cdot$ $10^{-4}$         & \ding{109}   \\ \hline
%            HEAX \cite{riazi_heax}   &       FPGA - Intel Arria10 GX 1150  & $2^{14}$ &         27  &         $582148$ / $1554005$ / $3986$ / $2018$ &   -                  &       300 &  1536       &     $\dagger$           & N/A   \\ \hline
%            Roy \cite{roy2019fpga}   &        Xilinx Zynq UltraScale+ ZCU102  &  $2^{12}$ &         30  &          $63522$ / $25622$ / $400$ / $200$ &   -                  &       200 & 16425       &      $\dagger$         & N/A    \\ \hline
%         %   Liu \cite{liu2019optimized}   &        20  & $2^{13}$ &         27  &          - &    -                  &      333 &  33966       &      -        & -    & \ding{109}    \\ \hline
%     \end{tabular}
%     }
%     % \vspace{1em}
%     \caption{Comparative table and performance of the NTT operation against related work}
%     % \caption{Performance comparison of the NTT operation against related work}
%     \footnotesize{$\dagger$ No information is available to accurately map FPGA resources to silicon area }\\
%     %\vspace{-0.4cm}
%     \label{tab:F1_HEAX_comp}
%     % \vspace{-0.4cm}
% \end{table*}


% % $^1$ Efficiency is measured in NTT operations per $ns$ per $mm^2$ $\cdot$ $10^{-4}$,

==> tables/io_ports.tex <==
\begin{table}[H]
    \centering
    \begin{tabular}{||l|c|l||}
        \hline
        \textbf{Pin Name} & $\rightarrow$ & \textbf{Description}                             \\ \hline \hline
        \multirow{2}*{CLK}               & \multirow{2}*{in}            & Reference clock    \\
                                         &                              & to PLL             \\ \hline
        \multirow{2}*{HOST\_IRQ}         & \multirow{2}*{out}           & External host      \\
                                         &                              & interrupt          \\ \hline
        nPORESET                         & in                           & Active low reset   \\ \hline
        SPIS\_CLK                        & in                           & SPI IO clock      \\ \hline
        SPIS\_CS                         & in                           & SPI Chip select     \\ \hline
        \multirow{2}*{SPIS\_MISO}        & \multirow{2}*{out}           & SPI MISO inter-    \\
                                         &                              & face for host read \\ \hline
        \multirow{2}*{SPIS\_MOSI}        & \multirow{2}*{in}            & SPI MOSI line      \\
                                         &                              & for host write     \\ \hline
        \multirow{2}*{UARTM\_TX}         & \multirow{2}*{out}           & UART TX line       \\
                                         &                              & for host read      \\ \hline
        \multirow{2}*{UARTM\_RX}         & \multirow{2}*{in}            & UART RX line       \\
                                         &                              & for host write     \\ \hline
        \multirow{3}*{UARTS\_TX}         & \multirow{3}*{out}           & UART TX line       \\
                                         &                              & for debug and      \\
                                         &                              & compute done       \\ \hline
    \end{tabular}
    \caption{Input/output ports. $\rightarrow$: direction.}
    \label{tab:io_ports}
\end{table}


% \begin{table}[H]
%     \centering
%     \begin{tabular}{||c|c|l||}
%         \hline
%         \multicolumn{1}{||c}{\textbf{$\rightarrow$}} & \multicolumn{1}{|c|}{\textbf{Pin Name}} & \multicolumn{1}{l||}{\textbf{Comments}} \\ \hline \hline
%         \multirow{6}*{in}                        & CLK                                   & Reference clock to PLL                        \\ %\cline{2-3}
%         {}                                       & nPORESET                              & Active low reset                              \\ %\cline{2-3}
%         {}                                       & SPIS\_CLK                             & SPI interface clock                           \\ %\cline{2-3}
%         {}                                       & SPIS\_CS                              & Chip select for SPI                           \\ %\cline{2-3}
%         {}                                       & SPIS\_MOSI                            & SPI MOSI line for host write                  \\ %\cline{2-3}
%         {}                                       & UARTM\_RX                             & UART RX line for host write                   \\ \hline
%         \multirow{3}*{out}                       & HOST\_IRQ                             & External Host interrupt                       \\ %\cline{2-3}
%         {}                                       & SPIS\_MISO                            & SPI MISO interface for host read              \\ %\cline{2-3}
%         {}                                       & UARTM\_TX                             & UART TX line for host read                    \\ \hline
%     \end{tabular}
%     \caption{Input/output ports. $\rightarrow$: direction.}
%     \label{tab:io_ports}
% \end{table}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{||c|c|l||}
%         \hline
%         \multicolumn{1}{||c}{\textbf{Direction}} & \multicolumn{1}{|c|}{\textbf{Pin Name}} & \multicolumn{1}{c||}{\textbf{Comments}}                \\ \hline \hline
%         \multirow{6}*{Input}                     & CLK                                   & Reference clock to PLL.                              \\ %\cline{2-3}
%         {}                                       & nPORESET                              & Active low reset.                                    \\ %\cline{2-3}
%         {}                                       & SPIS\_CLK                             & SPI interface clock.                                 \\ %\cline{2-3}
%         {}                                       & SPIS\_CS                              & Chip select for SPI.                                 \\ %\cline{2-3}
%         {}                                       & SPIS\_MOSI                            & SPI MOSI line for external host to write data        \\ %\cline{2-3}
%         {}                                       & UARTM\_RX                             & UART RX line for external host to write data.        \\ \hline
%         \multirow{3}*{Output}                    & HOST\_IRQ                             & External Host interrupt.                             \\ %\cline{2-3}
%         {}                                       & SPIS\_MISO                            & SPI MISO interface for external host to read result. \\ %\cline{2-3}
%         {}                                       & UARTM\_TX                             & UART TX line for external host to read result.       \\ \hline
%     \end{tabular}
%     \caption{Input/output ports.}
%     \label{tab:io_ports}
% \end{table}

==> tables/modules.tex <==
\begin{table}[b!]
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Module}} &  \multicolumn{1}{|c|}{\textbf{Color}}              \\ \hline
Multiplier Pool               & RED                                    \\ \hline
Cortex M0               & GREEN                              \\ \hline
SPIM           & BLUE 
   \\ \hline
DMA  & YELLOW
\\ \hline  
MDMC & PURPLE
\\ \hline
AHB & PEACH
\\ \hline
\end{tabular}
\caption{MODULES AND COLORS}
\label{tab:module_colors}
\end{table}

==> tables/notation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{r|l}
        \hline
        {\bf Symbol} & {\bf Description}   \\ \hline
                 $q$ & coefficient modulus \\
                 $n$ & polynomial degree   \\
            $n^{-1}$ & inverse of $n$ ($n \cdot n^{-1} \equiv 1 \mod q$) \\
            $\Omega$ & twiddle factors     \\
           $\lambda$ & length (bytes)      \\ \hline
    \end{tabular}
    \caption{Notation.}
    \label{tab:notation}
\end{table}

==> tables/opt_scenarios.tex <==
% \begin{table}[b!]
% \begin{tabular}{|l|l|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Scenario}} &  \multicolumn{1}{|c|}{\textbf{Analysis Type}}     \\ \hline
% std\_max\_ss\_nominal\_max\_1p08v\_125c\_cmax & setup
% \\ \hline
% std\_max\_tt\_nominal\_max\_1p20v\_25c\_cmax &
% setup
% \\ \hline
% std\_min\_ff\_nominal\_min\_1p32v\_m40c\_cmin &
% hold
% \\ \hline
% std\_min\_tt\_nominal\_max\_1p20v\_25c\_cmin &
% hold
% \\ \hline
% std\_min\_fff\_nominal\_min\_1p32v\_125c\_cmin &
% hold 
% \\ \hline
% \end{tabular}
% \caption{Optimisation scenarios and analysis types }
% \label{tab:scenarios}
% \end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{||l|l||}
        \hline
        \multicolumn{1}{||c|}{\textbf{Scenario}}         & \multicolumn{1}{c||}{\textbf{Analysis Type}} \\ \hline \hline
        std\_max\_ss\_nominal\_max\_1p08v\_125c\_cmax  & \multirow{2}*{setup}                       \\
        std\_max\_tt\_nominal\_max\_1p20v\_25c\_cmax   & {}                                         \\ \hline
        std\_min\_ff\_nominal\_min\_1p32v\_m40c\_cmin  & \multirow{3}*{hold}                        \\
        std\_min\_tt\_nominal\_max\_1p20v\_25c\_cmin   & {}                                         \\
        std\_min\_fff\_nominal\_min\_1p32v\_125c\_cmin & {}                                         \\ \hline
    \end{tabular}
    \caption{Optimization scenarios and analysis types.}
    \label{tab:scenarios}
    % \vspace{-1.1cm}
\end{table}

==> tables/parameters.tex <==
% Table of recommended encryption parameters according to the Homomorphic Encryption Security Standard

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale = 1]{figs/encryption_parameters.png}
%     \caption{Table of recommended encryption parameters \cite{hestd}.}
%     \label{tab:parameters}
% \end{figure}

\begin{table}[t]
    \centering
    \begin{tabular}{||c|c|rrrrrr||}
        \hline
        {cost}  & {} & \multicolumn{6}{c||}{$n$} \\
        {model} & $\lambda$ & $2^{10}$ & $2^{11}$ & $2^{12}$ & $2^{13}$ & $2^{14}$ & $2^{15}$ \\ \hline \hline
        \multirow{3}*{BKZ.sieve}  & 128 &  27 &  54 & 109 & 218 & 438 & 881 \\
        {}                        & 192 &  19 &  37 &  75 & 152 & 305 & 611 \\
        {}                        & 256 &  14 &  29 &  58 & 118 & 237 & 476 \\ \hline
        \multirow{3}*{BKZ.qsieve} & 128 &  25 &  51 & 101 & 202 & 411 & 827 \\
        {}                        & 192 &  17 &  35 &  70 & 141 & 284 & 571 \\
        {}                        & 256 &  13 &  27 &  54 & 109 & 220 & 443 \\ \hline
    \end{tabular}
    \vspace{1em}
    \caption{Table of recommended encryption parameters ($\log q$) assuming access to a classical computer only (BKZ.sieve) or a quantum computer (BKZ.qsieve) for different polynomial degrees $n$ and security levels $\lambda$ \cite{hestd}.}
    \label{tab:parameters}
\end{table}
% \vspace{-2em}

==> tables/related_work.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{||c|c|c|c|c|c|c|c|c||}
        \hline
         \multirow{2}*{\bf Design} & {\bf Node} &  {\bf n} & {\bf log q} & {\bf Area} & {\bf Area} & {\bf Freq.} &         {\bf Power} & \multirow{2}*{\bf Fab.} \\
                                {} &     ($nm$) &          &    ($bits$) &   ($mm^2$) & ($kgates$) &     ($Mhz$) &               ($W$) & {}                      \\ \hline \hline
                         \cofhee{} &         55 & $2^{14}$ &         128 &         12 &          - &         250 &  $2.3 \cdot 10^{-2}$ & \ding{108}              \\ \hline
               \cite{tan2021ultra} &         32 & $2^{12}$ &         32 &       57.1 &          - &           -  & $2.3 \cdot 10^{-2}$ & \ding{109}              \\ \hline
             \cite{feldmann2021f1} &      14/12 & $2^{14}$ &         32  &      151.4 &          - &        1000 &    $1.8 \cdot 10^2$ & \ding{109}              \\ \hline
           \cite{tan2019efficient} &         32 & $2^{12}$ &         32 &          - &       6.54 &           -  &                   - & \ding{109}              \\ \hline
    \end{tabular}
    }
    % \vspace{1em}
    \caption{Related work of ASIC designs}
    % \caption{Related work of ASIC designs of FHE accelerators. $n$ stands for the maximum polynomial degree, while $\log q$ represents the maximum modulus size natively supported by the hardware (i.e. without requiring RNS)}
    \vspace{-0.3cm}
    \label{tab:related_designs}
    % \vspace{-0.4cm}
\end{table}


==> tables/synthesis.tex <==
\begin{table}[t]
    \centering
    \caption{Post-synthesis area and timing estimations.}
    \begin{tabular}{||l|r|c||}
         \hline
         \multirow{2}{*}{\parbox{2.0cm}{{\bf Blocks}}}                      &
         \multirow{2}{*}{\parbox{1.4cm}{\centering {\bf Area $({um}^2)$}}}                        &
         \multirow{2}{*}{\parbox{2.0cm}{\centering {\bf Worst path delay $(ns)$}}}                        \\
         {} & {} & {}  \\
         \hline \hline
         %\textbf{Blocks} & \textbf{Area in $um^2$} & \textbf{Worst Path Delay in  $ns$}\\ \hline \hline
         ARM Cortex M0                      & 35,422     & 5.24 \\ \hline
         MDMC                               & 27,281     & 4.16  \\ \hline
         PE                                 & 639,387    & 5.65  \\ \hline
         DMA                                & 7,545      & 7.17  \\ \hline
         SPI                                & 20,024     & 7.74  \\ \hline
         UART-M                             & 3,467      & 5.66  \\ \hline
         AHB bus                            & 74,692     & 5.76  \\ \hline
         GPCFG                              & 53,374     & 7.03 \\ \hline
         UART-S                             & 3,005      & 4.93 \\ \hline
         Dual-port SRAM                     & 1,783,551  & 4.22 \\ \hline
         Single-port SRAM                   & 800,904    & 4.19 \\ \hline
    \end{tabular}
    \label{tab:synthesis}
\end{table}
